Characterizing Browser Fingerprinting and its Mitigations

People are becoming increasingly concerned with their online privacy, especially with how advertising companies track them across websites (a practice called cross-site tracking), as reconstructing a user's browser history can reveal sensitive information. Recent legislation like the General Data Protection Regulation (GDPR) and the California Consumer Privacy Act have tried to limit the extent to which third parties perform cross-site tracking, and browsers have also made tracking more difficult by deprecating the most-common tracking mechanism: third-party cookies. However, online advertising companies continue to track users through other mechanisms that do not rely on cookies. This work explores one of these tracking techniques: browser fingerprinting. We detail how browser fingerprinting works, how prevalent it is, and what defenses can mitigate it.

==> Makefile <==
SHELL := /bin/bash

extensions_to_clean := out aux log bbl blg fls fdb_latexmk glg gls lof glo glsdefs lot toc dvi ist acn acr synctex.gz alg xdy

all: main

clean:
	@if [[ -f paper.pdf ]]; then \
		rm paper.pdf;\
	fi;
	@for extension in $(extensions_to_clean); do \
		find . -type f -name "*.$$extension" -delete;\
	done;
	@rm -f diff.*

main:
	latexmk -bibtex -pdf paper
	pdflatex -bibtex -interaction=batchmode paper

diff:
	latexmk -bibtex -pdf diff
	pdflatex -bibtex -interaction=batchmode diff


==> content/conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}

==> content/http-request-header.tex <==
\begin{table*}[]
    \begin{tabular}{|l|l|l|}
    \hline
    HTTP Request Header & HTTP Request Header Value & Notes \\ \hline
    Accept & text/html,application/xhtml+xml,... &  \\ \hline
    Accept-Encoding & gzip, deflate, br &  \\ \hline
    Accept-Language & en-US,en;q=0.9,da;q=0.8,es;q=0.7 &  \\ \hline
    Connection & keep-alive &  \\ \hline
    Cookie & {[}omitted for length{]} &  \\ \hline
    DNT & 1 & "Do Not Track" \\ \hline
    Host & cse.ucsd.edu &  \\ \hline
    sec-ch-ua & "Google Chrome";v="105", "Not)A;Brand";v="8", "Chromium";v="105" &  \\ \hline
    sec-ch-ua-mobile & ?0 &  \\ \hline
    sec-ch-ua-platform & "macOS" &  \\ \hline
    Sec-Fetch-Dest & document &  \\ \hline
    Sec-Fetch-Mode & navigate &  \\ \hline
    Sec-Fetch-Site & none &  \\ \hline
    Sec-Fetch-User & ?1 &  \\ \hline
    sec-gpc & 1 &  \\ \hline
    Upgrade-Insecure-Requests & 1 &  \\ \hline
    User-Agent & \begin{tabular}[c]{@{}l@{}}Mozilla/5.0 (Macintosh; Intel Mac OS X 10\_15\_7) AppleWebKit/537.36\\ (KHTML, like Gecko) Chrome/105.0.0.0 Safari/537.36\end{tabular} &  \\ \hline
    \end{tabular}
    \caption{An example of the HTTP Request headers for a request to load cse.ucsd.edu.}
    \label{tab:http-request-header}
    \end{table*}
